Optimal Controller Realizations against False Data Injections in Cooperative Driving

To enhance the robustness of cooperative driving to cyberattacks, we study a controller-oriented approach to mitigate the effect of a class of False-Data Injection (FDI) attacks. By reformulating a given dynamic Cooperative Adaptive Cruise Control scheme (the base controller), we show that a class of new but equivalent controllers (base controller realizations) can represent the base controller. This controller class exhibits the same platooning behavior in the absence of attacks, but in the presence of attacks, their robustness varies with the realization. We propose a prescriptive synthesis framework where the base controller and the system dynamics are written in new coordinates via an invertible coordinate transformation on the controller state. Because the input-output behavior is invariant under coordinate transformations, the input-output behavior is unaffected (so controller realizations do not change the system's closed-loop performance). However, each controller realization may require a different combination of sensors. Subsequently, we obtain the optimal combination of sensors that minimizes the effect of FDI attacks by solving a linear matrix inequality while quantifying the FDI's attack impact through reachability analysis. Through simulation studies, we demonstrate that this approach enhances the robustness of cooperative driving without relying on a detection scheme and maintaining all system properties.

==> 3_ProblemSetting/3.99_ModelDescription.tex <==
 The controller in \cite{Ploeg2014a} is a dynamic controller of the following form:
\begin{equation}
\label{eq:Controller0}
    \mathcal{C} \coloneqq \dot{u}_i = -\tfrac{1}{h} u_i + \tfrac{k_p}{h} e_i + \tfrac{k_d}{h} \dot{e}_i + \tfrac{k_{dd}}{h} \ddot{e}_i + \tfrac{1}{h}u_{i-1}, 
\end{equation}
where $k_p, k_d$, and $k_{dd}$ are the controller gains. We refer to $\mathcal{C}$ as the base controller.

The real-time realization of any control scheme depends on the available sensors $y_{i,j}$ (sensor number $j$ of vehicle $i$). We use sensor data from onboard sensors (e.g., radar, LiDAR, cameras, and velocity/acceleration sensors) and receive data transmitted wirelessly between adjacent vehicles. We assume that the sensors available to implement control actions are:
\begin{subequations}
\label{eq:SensorMeasurements}
    \begin{align}
        y_{i,1} &\coloneqq q_{i-1}(t) - q_{i}(t) - L_i + \delta_{i,1}(t), \\
        y_{i,2} &\coloneqq v_i(t) + \delta_{i,2}(t), \\
        y_{i,3} &\coloneqq a_i(t) + \delta_{i,3}(t), \\
        y_{i,4} &\coloneqq v_{i-1}(t) - v_i(t) + \delta_{i,4}(t), \\
        y_{i,5} &\coloneqq a_{i-1}(t) + \delta_{i,5}(t), \\
        y_{i,6} &\coloneqq u_{i-1}(t) + \delta_{i,6}(t).
    \end{align}
\end{subequations}
Herein, $\delta_{i,j}(t)$ models potential false data injection attacks and $j \in \{1, ..., 6\}$. It is important to note that sensors $y_{i,1}$ and $y_{i,4}$ provide relative tracking and relative velocity information, $y_{i,2}$ and $y_{i,3}$ are the onboard measured velocity and acceleration, and sensors $y_{i,5}$ and $y_{i,6}$ model data received wirelessly from the preceding vehicle via V2V communication. Using the measured values in \eqref{eq:SensorMeasurements}, base controller \eqref{eq:Controller0} can be implemented as follows:
\begin{align}\label{eq:ui1}
&\mathcal{C}_1 \coloneqq \left\{ 
    \begin{aligned}
        \dot{\xi}_{i,1} &= -(\tfrac{1}{h} + \tfrac{k_{dd}}{\tau})\xi_{i,1} + \tfrac{k_p}{h} y_{i,1} - k_p y_{i,2} \\ 
                        & \,\,\,\,\,\,\, - (k_d + \tfrac{k_{dd}}{h} - \tfrac{k_{dd}}{\tau}) y_{i,3} + \tfrac{k_d}{h}y_{i,4} \\
                        & \,\,\,\,\,\,\, + \tfrac{k_{dd}}{\tau}y_{i,5} + \tfrac{1}{h} y_{i,6} - \tfrac{k_p}{h} r_i \\
        {u}_{i} &= {\xi}_{i,1},
    \end{aligned} \right.
\end{align}
with controller state $\xi_{i,1} \in \mathbb{R}$. 

We remark that the controller implementation in \eqref{eq:ui1} is not unique and refer to such a controller as a realized controller. An infinite number of equivalent realizations of the base controller $\mathcal{C}$ exist that result in the same control signal $u_i(t)$ at the vehicle for $\delta_{i,j} = 0$. For instance, consider the CACC controller in \cite{Lefeber2020}, with a change of coordinates $\tfrac{\tau}{h}\xi_{i,2} = \tfrac{\tau}{h}a_{i-1} + (1-\tfrac{\tau}{h})a_i - \xi_{i,1}$ and new controller state $\xi_{i,2} \in \mathbb{R}$. Applying this coordinate transformation to \eqref{eq:Controller0}, and using the available sensors in \eqref{eq:SensorMeasurements}, a second realized controller, $\mathcal{C}_2$, can be obtained as
\begin{align}\label{eq:ui2}
&\mathcal{C}_2 \coloneqq \left\{ 
    \begin{aligned}
        \dot{\xi}_{i,2} &= -\tfrac{1+k_{dd}}{\tau}\xi_{i,2} - \tfrac{k_p}{\tau} y_{i,1} + \tfrac{k_p h}{\tau} y_{i,2} \\ 
                        & \,\,\,\,\,\,\, + \tfrac{k_{d} h}{\tau} y_{i,3} - \tfrac{k_d}{\tau}y_{i,4} + \tfrac{k_p}{\tau} r_i, \\
        {u}_{i} &= \tfrac{\tau}{h}y_{i,5} + (1 - \tfrac{\tau}{h})y_{i,3} - \tfrac{\tau}{h}\xi_{i,2}.
    \end{aligned} \right.
\end{align}
That is, we have two different realizations, $\mathcal{C}_1$ and $\mathcal{C}_2$, of the CACC controller in \eqref{eq:Controller0} --- each result in the same control signal $u_i(t)$ applied to the vehicle for $\delta_{i,j}(t) = 0$. Note that $\mathcal{C}_2$ requires the actual acceleration of the preceding vehicle, whereas $\mathcal{C}_1$ requires the control input of the preceding vehicle. However, when $\delta_{i,j}(t) \neq 0$, for some $t\geq 0$, they will, in general, lead to different control signals $u_i(t)$.

To quantify the impact of the attack on the two different controller realizations, we are interested in the reachable sets induced by the attack signals $\delta_{i,j}(t)$ and use the size of these sets as a security metric. Here, we are interested in assessing whether $\mathcal{C}_1$ and $\mathcal{C}_2$ lead to different sensitivity to attacks for the same class of resource-limited adversaries for varying system and control parameters. 


%Both $\mathcal{C}_1$ and $\mathcal{C}_2$ are evaluated by computing the adversarial reachable sets for varying system and control parameters, where a difference in size indicates a more resilient implementation. 

%\begin{equation}
%\label{eq:Controller0}
%    \mathcal{C} \coloneqq \left\{
%    \!\begin{aligned}%[b]
%        \dot{\eta}_i &= -\tfrac{1}{h} \eta_i + \tfrac{k_p}{h} e_i + \tfrac{k_d}{h} \dot{e}_i + \tfrac{k_{dd}}{h} \ddot{e}_i + \tfrac{1}{h}u_{i-1}, \\
%        u_i &= \eta_i,
%    \end{aligned} \right.
%\end{equation}

==> 4_Approach/4.1_LinearCoordinateTransformationV2.tex <==
\subsection{Controller Realization} \vspace{-1mm}
One could interpret the difference between the CACC controllers in \eqref{eq:SD_BaseController} and \eqref{eq:C2_Lefeber} as a coordinate transformation on the internal control variable from $\rho_i$ to $\hat{\rho}_i$. Therefore, we propose to find the class of controllers that yields the same control signal $u_i$ by applying the following coordinate transformation 
%\begin{align} \label{eq:CR_Transformation} \begin{split}
%   \! \! \! \! \bar{\rho}_i &= \alpha_i \rho_i + \beta_1 y_{i,1} + \beta_2 y_{i,2} + \beta_3 y_{i,3} + \beta_4 y_{i,4} + \beta_5 y_{i,5}, \\
%                               \alpha_i \rho_i + \beta_1 y_{i,1} + \beta_2 y_{i,2} + \beta_3 y_{i,3} + \beta_4 y_{i,4} + \beta_5 y_{i,5},
%\end{split}\end{align}
\begin{align} \label{eq:CR_Transformation}
  \bar{\rho}_i &= \alpha_i \rho_i + \underbrace{\begin{bmatrix} \beta_{i,1} & \beta_{i,2} & \beta_{i,3} & \beta_{i,4} & \beta_{i,5} & 0 \end{bmatrix}}_{\beta_i} y_i,
\end{align}
with new controller state $\bar{\rho}_i$. The goal is to determine the optimal values for both $\alpha_i \in \mathbb{R}$ and $\beta_i\in \mathbb{R}^{n_y - 1}$ ($n_y$ number of measurements) to reduce the impact of FDI attacks. Note that in the coordinate transformation $\beta_{i,6} = 0$ (excluding $y_{i,6}$), as this would require information about $\dot{u}\imo$ in the transformed dynamics, and thus also knowledge about the control structure of vehicle $i-1$ (and possibly sensor data from vehicle $i-2$).

For the closed-loop system, the formulation of \cite{lefeber_cooperative_2020} is adopted, where it was observed that the resulting closed-loop dynamics, with output $e_i$ and input $u_i$, has relative degree two. Therefore, we differentiate the output $e_i$ twice and then investigate the resulting internal dynamics. To this end, we define the stacked state vector $x = [ e_i \ \dot{e}_i \ z_i \ \vim \ \aim ]^\top$, where $z_i \! \coloneqq \! \vim - v_i$ is the internal dynamic state, which is input-to-state stable with respect to $\aim$ \cite{lefeber_cooperative_2020}. Using \eqref{eq:SD_PlatoonDynamics} and \eqref{eq:SD_ErrorFormulation} we obtain the platooning dynamics of the form:
\begin{align} \label{eq:CR_CL_Form}
    \! \! \! \! \begin{bmatrix} 
    \dot{x}_i \\ 
    \dot{x}\imo
    \end{bmatrix} 
    &= \begin{bmatrix}
        A_{11} & A_{12} \\ 
        A_{21} & A_{22}
    \end{bmatrix} 
    \begin{bmatrix} 
    x_i \\ 
    x\imo
    \end{bmatrix}+ 
    \begin{bmatrix} B_1 & 0 \\ 0 & B_2 \end{bmatrix} \begin{bmatrix} u_i \\ \uim \end{bmatrix},
\end{align}
where
\small{\begin{align} \label{eq:RC_CL_Matrices}
   \! \! \! \! \! A \! &= \! \! 
    \left[ \begin{array}{ccc|cc}
        0               & 1                                 & 0                                     & 0             & 0 \\ 
        0               & \tfrac{1}{h} - \tfrac{1}{\tau}      & \tfrac{1}{\tau} -\frac{1}{h}           & 0             & 1 \\ 
        0               & \tfrac{1}{h}                       & -\tfrac{1}{h}                          & 0             & 1 \\ \hline
        0               & 0                                 & 0                                     & 0             & 1 \\ 
        0               & 0                                 & 0                                     & 0             & -\tfrac{1}{\tau}
    \end{array}\right] \! \!,
    B \! = \! \!
    \left[ \begin{array}{c|c}
     0                  & 0\\ 
     -\tfrac{h}{\tau}   & 0 \\ 
     0                  & 0 \\ \hline           
     0                  & 0 \\ 
     0                  & \tfrac{1}{\tau}
    \end{array} \right] \! \!,
\end{align}} \normalsize{}
and by substituting the base controller from \eqref{eq:SD_BaseController} we obtain:
\begin{align} \label{eq:RC_CL_Base}
    \begin{bmatrix}
        \dot{x} \\ \dot{\rho}_i
    \end{bmatrix} &= 
    \underbrace{\begin{bmatrix}
        A & B_1 \\
        K & -\tfrac{1}{h}
    \end{bmatrix}}_{\mathcal{A}} 
    \begin{bmatrix}
        x \\ \rho_i
    \end{bmatrix} + 
    \underbrace{\begin{bmatrix}
        B_2 \\ \tfrac{1}{h}
    \end{bmatrix}}_{\mathcal{B}_{\uim}} \uim, 
\end{align}  \vspace{-0mm}
as the closed-loop dynamics, where $K = [\tfrac{k_p}{h} \ \ \tfrac{k_d}{h} \ \ 0 \ \ 0 \ \ 0]$.

The sensor measurements in \eqref{eq:SD_Sensors} can be expressed in terms of the closed-loop coordinates and disturbance $\uim$, as the coordinate transformation from $[ d_i \ v_i \ a_i \ \vim \ \aim]^\top$ to $[ e_i \ \dot{e}_i \ z_i \ \vim \ \aim]^\top$ is invertible. For $\delta_{i}=0$, we obtain
\begin{align} \label{eq:CR_SensorError}
    y_i &= 
    \underbrace{\begin{bmatrix}
        1 & 0 & -h_{i} & h_{i} & 0 \\ 
        0 & 0 & -1 & 1 & 0 \\ 
        0 & -\tfrac{1}{h} & \tfrac{1}{h} & 0 & 0 \\ 
        0 & 0 & 1 & 0 & 0 \\ 
        0 & 0 & 0 & 0 & 1 \\ 
        0 & 0 & 0 & 0 & 0
    \end{bmatrix}}_{C}
    \begin{bmatrix}
        e_i \\ \dot{e}_i \\ z_i \\ \vim \\ \aim
    \end{bmatrix} + 
    \underbrace{\begin{bmatrix}
        0 \\ 0 \\ 0 \\ 0 \\ 0 \\ 1
    \end{bmatrix}}_{D} \uim.
\end{align}
Given that $(C, \ D )$ is full rank, \eqref{eq:CR_SensorError} can be rewritten as
\begin{align} \label{eq:InverseSensor}
    \begin{bmatrix}
        x \\ \uim
    \end{bmatrix} &= [C \ \ D ]^{-1} y_i.
\end{align}

To derive the class of base controller realizations,  $\dot{\rho}_i$ in \eqref{eq:SD_BaseController} is first reformulated using the proposed change of coordinates in \eqref{eq:CR_Transformation} and subtituting \eqref{eq:InverseSensor}, resulting in
\begin{align} \label{eq:RC_drho} \begin{split}
    \dot{\rho}_i &= -\tfrac{1}{\alpha_i h}\bar{\rho}_i + \left([ K \ \ \tfrac{1}{h} ] [C \ \ D ]^{-1} + \tfrac{1}{\alpha_i h} \beta_i\right) y_i.
\end{split} \end{align}
The dynamics of $\bar{\rho}_i$ are then obtained by differentiating \eqref{eq:CR_Transformation},
\begin{align} \begin{split}
    \dot{\bar{\rho}}_i &= \alpha_i \dot{\rho}_i + \beta_i \dot{y}_i \\
                     &= \alpha_i \dot{\rho}_i + \beta_i (C \dot{x} + D \dot{u}\imo),
\end{split}\end{align}
where due to the structure of $\beta_i$ and $D$ we have that $\beta_i D = 0$. Substitution of \eqref{eq:CR_CL_Form} and \eqref{eq:InverseSensor} provides that
\begin{align}\label{eq:RC_drho_bar1} \begin{split}
    \dot{\bar{\rho}}_i &= \alpha_i \dot{\rho}_i + \beta_i C [ A \ \ B_2 ] [C \ \ D ]^{-1} y_i  + \beta_i C B_1 u_i.
\end{split}\end{align}
The new formulation of the control input $u_i$ is obtained by applying the change of coordinates to \eqref{eq:SD_BaseController}, resulting in
\begin{subequations} \label{eq:RealizationClass}   
\begin{align} \label{eq:RC_ui}
    u_i \! &= \! \tfrac{1}{\alpha_i} \bar{\rho}_i - \tfrac{1}{\alpha_i} \beta_i y_i. 
\intertext{Substitution of \eqref{eq:RC_drho} and \eqref{eq:RC_ui} into \eqref{eq:RC_drho_bar1} yields}
\begin{split} \label{eq:RC_drho_bar2} 
     \dot{\bar{\rho}}_i &= (\tfrac{1}{\alpha_i} \beta_i C B_1  -\tfrac{1}{h}) \bar{\rho}_i + \left( \left( \alpha_i [ K \ \ \tfrac{1}{h} ] + \right. \right. \\ 
    & \left. \left. \beta_i C [ A \ \ B_2 ] \right) [ C \ \ D ]^{-1}  
    \! \! + \! \tfrac{1}{h} \beta_i \! - \! \tfrac{1}{\alpha_i} \beta_i C B_1 \beta_i \right) y_i.
\end{split}\end{align}
\end{subequations}
Consequently, \eqref{eq:RealizationClass} represents the class of equivalent controller realizations of \eqref{eq:SD_BaseController}, which exhibit equivalent platooning behavior in the absence of an FDI attack. Notice that for $\alpha_i = 1, \beta_i = 0$, and for $\alpha_i = -\tfrac{\tau}{h}, \beta_i = [0 \ \ 0 \ \ (1-\tfrac{\tau}{h}) \ \ 0 \ \ \tfrac{\tau}{h} \ \ 0]$, the controller realizations $\mathcal{C}$ and $\hat{\mathcal{C}}$ are obtained, respectively. To this end, \eqref{eq:RealizationClass} is derived for $\delta_i = 0$ to find all equivalent controller realizations that exhibit the same platooning behavior in the absence of FDI attacks. However, the change of coordinates affects the combinations of sensors being used and, therefore, also influences the effect of an FDI on the platooning behavior. To model the effect of FDI attacks, we now derive \eqref{eq:RealizationClass} for $\delta_i \neq 0$ by reformulating \eqref{eq:CR_SensorError} 
\begin{align} \label{eq:CR_y_att}
    y_i &= [C \ \ D ] \begin{bmatrix}
        x \\ \uim
    \end{bmatrix} + \delta_i.
\end{align}
Substitution of \eqref{eq:CR_y_att} into \eqref{eq:RealizationClass} yields the realized controller in presence of attacks, 
\begin{subequations} \label{eq:RealizedController} \begin{align}
    u_i \! &= \! \tfrac{1}{\alpha_i} \bar{\rho}_i - \tfrac{1}{\alpha_i} \beta_i [C \ \ D ] \begin{bmatrix} x \\ \uim \end{bmatrix} - \tfrac{1}{\alpha_i} \beta_i \delta_i, \\
    \begin{split} 
        \dot{\bar{\rho}}_i \! &= \! (\tfrac{1}{\alpha_i} \beta_i C B_1  -\tfrac{1}{h}) \bar{\rho}_i + \left( \alpha_i [ K \ \ \tfrac{1}{h} ] + \beta_i C [ A \ \ B_2 ] \right. \\
        & \ \ \left. + (\tfrac{1}{h} \beta_i -\tfrac{1}{\alpha_i} \beta_i C B_1 \beta_i)[C \ \ D ] \right) \begin{bmatrix} x \\ \uim \end{bmatrix} \\
        & \ \ + \left( \left( \alpha_i [ K \ \ \tfrac{1}{h} ] + \beta_i C [ A \ \ B_2 ] \right) [C \ \ D ]^{-1}  \right. \\
        & \ \ \left. + \tfrac{1}{h} \beta_i - \tfrac{1}{\alpha_i} \beta_i C B_1 \beta_i \right) \delta_i.
\end{split}\end{align}\end{subequations}
When deriving the closed-loop system using \eqref{eq:RealizedController}, the system matrices $\bar{\mathcal{A}}(\alpha_i, \beta_i)$ and $\bar{\mathcal{B}}_{\uim}(\alpha_i, \beta_i)$ are dependent on the choice of $\alpha_i$ and $\beta_i$. Although different sensors are used, the realization does not affect the nominal closed-loop behavior, as the input-output behavior in the absence of FDI attacks is invariant under a linear coordinate transformation, also known as a similarity transformation. Therefore, after selecting the required combination of sensors (including $\delta_i$), the closed-loop system is transformed back to its original coordinates $[x \ \ \rho_i]^\top$. As a result: (i) a fair analysis is made between different realizations, as $\mathcal{{A}}$ and $\mathcal{B}_{\uim}$ are independent, and only $\mathcal{B}_{\delta_i}$ is dependent on $\alpha_i$ and $\beta_i$, and (ii) the resulting dynamics are affine in $\tfrac{1}{\alpha_i}\beta_i$, allowing for linear and convex optimization techniques, whereas solving it in the new coordinates requires nonlinear optimization techniques. To prove the latter, note that the change of coordinates in \eqref{eq:CR_Transformation} is invertible for $\alpha \neq 0$:
\begin{align}
\begin{bmatrix}
        x \\ \bar{\rho}_i
    \end{bmatrix}&=
    \begin{bmatrix}
        I & 0 \\
        \beta_iC & \alpha_i
    \end{bmatrix} \begin{bmatrix}
        x \\ \rho_i
    \end{bmatrix}.
\end{align}
By applying the inverse coordinate transformation to the closed-loop system \eqref{eq:RealizedController}, the original closed-loop system \eqref{eq:RC_CL_Base} is obtained, including a matrix that maps a potential FDI attack onto the closed-loop system
\begin{subequations}
   \begin{align} \label{eq:RC_CL_Att}
    \begin{bmatrix}
        \dot{x} \\ \dot{\rho}_i
    \end{bmatrix} &= 
    \mathcal{A} 
    \begin{bmatrix}
        x \\ \rho_i
    \end{bmatrix} + 
    \mathcal{B}_{\uim} \uim + \mathcal{B}_{\delta_i} \delta_i,
\end{align}
where
\begin{align}
 \label{eq:RC_Bdelta}
    \! \!  \! \! \mathcal{B}_{\delta_i} \! &= \! \! 
    \begin{bmatrix}
        -\tfrac{1}{\alpha_i} B_1 \beta_i \\
        \left([ K \ \ \tfrac{1}{h} ] \! + \! \tfrac{1}{\alpha_i} \beta_i C [ A \ \ B_2 ]\right) \! [C \ \ D ]^{-1} \! \! + \tfrac{1}{h \alpha_i} \beta_i
    \end{bmatrix} \! \!.
\end{align}
\end{subequations}

Note that when converting the system back to its original coordinates, only the attack matrix $\mathcal{B}_{\delta_i}$ is affected by the choice of $\alpha_i$ and $\beta_i$. The following section introduces an optimization scheme to find the optimal realization of the base controller within the suggested class of realized controllers. 






